Query Complexity of Learning Axis-Aligned Partitions

This work establishes the query complexity of learning high-dimensional boxes in the exact query learning setting. Let $X \subset \mathbb{R}^d$ be a set of $n$ points, labeled by a collection of $k$ boxes: the label of each point in $X$ is determined by the unique box containing it. A learner aims to exactly recover the labels for every point in $X$ given access to a label oracle. We consider three increasingly-structured settings. In the most general setting, there are no conditions on the boxes, and they may overlap. We show that CAL (Cohn-Atlas-Ladner 1994), a classical active learning algorithm, is minimax-optimal with query complexity $\Theta(kd \log (n/kd))$. When the boxes are disjoint, we examine two regimes. In the large-$k$ regime, CAL remains minimax-optimal. For the constant-$k$ regime, an optimized variant of the Halving algorithm (Heged\"{u}s 1995) can beat CAL by a $\log(d)$ factor. Finally, in the most-structured settings, the boxes correspond to the leaves of a constant-sized decision tree. We prove a tight query complexity of $\Theta(d + \log n)$ that is additive in $d$ and $\log n$, generalizing a recent result (Black-Larsen-Mazumdar-Saha-So 2026) that establishes the query complexity of learning decision stumps.

==> figures/disjoint-2d.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[>=Latex, font=\small]
  % Panel (a): cube and coherent edge orders.
  \begin{scope}
    \node[font=\bfseries] at (1.35,3.35) {(a) Coherent edge orders};
    \draw[line width=0.8pt, gray!75] (0,0) -- (2.7,0) -- (2.7,2.2) -- (0,2.2) -- cycle;
    \draw[densely dashed, gray!55] (0,0) -- (2.7,2.2);
    \draw[densely dashed, gray!55] (0,2.2) -- (2.7,0);

    \node[circle, draw=RoyalBlue, fill=RoyalBlue!18, minimum size=8mm] (v00) at (0,0) {$00$};
    \node[circle, draw=BurntOrange, fill=BurntOrange!22, minimum size=8mm] (v10) at (2.7,0) {$10$};
    \node[circle, draw=ForestGreen, fill=ForestGreen!18, minimum size=8mm] (v01) at (0,2.2) {$01$};
    \node[circle, draw=Plum, fill=Plum!22, minimum size=8mm] (v11) at (2.7,2.2) {$11$};

    \draw[->, thick, MidnightBlue] (-0.65,0.25) -- (-0.65,1.95)
      node[midway,left] {$\prec_1$};
    \draw[->, thick, MidnightBlue] (2.45,2.85) -- (0.25,2.85)
      node[midway,above] {$\prec_2$};

    \node[align=left, font=\scriptsize] at (1.35,-1.02) {$
      (00\!-!10)\prec_1(01\!-!11)$\\[-1pt]
      $(10\!-!11)\prec_2(00\!-!01)$};
  \end{scope}

  % Panel (b): exact R^2 realization, using logical coordinates scaled to cm.
  \begin{scope}[shift={(7.75,0.35)}, x=0.205cm, y=0.205cm]
    \node[font=\bfseries] at (0,15.2) {(b) Boxes, anchors, and edge chains};

    % Boxes: L=3, A=6, C=12, thresholds (2,1,2,1).
    \filldraw[fill=RoyalBlue!18, draw=RoyalBlue!80!black, line width=0.6pt]
      (-12,-12) rectangle (2.3333,8.3333);
    \filldraw[fill=BurntOrange!22, draw=BurntOrange!85!black, line width=0.6pt]
      (2.6667,-12) rectangle (12,1.3333);
    \filldraw[fill=ForestGreen!18, draw=ForestGreen!75!black, line width=0.6pt]
      (-12,8.6667) rectangle (7.3333,12);
    \filldraw[fill=Plum!22, draw=Plum!80!black, line width=0.6pt]
      (7.6667,1.6667) rectangle (12,12);

    \node[font=\bfseries] at (-5.2,-2.6) {$B_{00}$};
    \node[font=\bfseries] at (7.2,-5.2) {$B_{10}$};
    \node[font=\bfseries] at (-2.5,10.2) {$B_{01}$};
    \node[font=\bfseries] at (9.8,6.3) {$B_{11}$};

    % Axes and frame.
    \draw[black!55, ->] (-13,0) -- (13.2,0) node[right] {$x_1$};
    \draw[black!55, ->] (0,-13) -- (0,13.2) node[pos=0.93,right] {$x_2$};
    \draw[black!70, line width=0.45pt] (-12,-12) rectangle (12,12);

    % Threshold-gap marks.
    \draw[densely dashed, black!70] (2.5,-12.8) -- (2.5,-11.2);
    \draw[densely dashed, black!70] (7.5,11.2) -- (7.5,12.8);
    \draw[densely dashed, black!70] (-12.8,8.5) -- (-11.2,8.5);
    \draw[densely dashed, black!70] (11.2,1.5) -- (12.8,1.5);

    % Fixed edge-chain points.
    \fill[RoyalBlue] (1,-12) circle[radius=2.2pt];
    \fill[RoyalBlue] (2,-12) circle[radius=2.2pt];
    \fill[BurntOrange] (3,-12) circle[radius=2.2pt];

    \fill[ForestGreen] (7,12) circle[radius=2.2pt];
    \fill[Plum] (8,12) circle[radius=2.2pt];
    \fill[Plum] (9,12) circle[radius=2.2pt];

    \fill[RoyalBlue] (-12,7) circle[radius=2.2pt];
    \fill[RoyalBlue] (-12,8) circle[radius=2.2pt];
    \fill[ForestGreen] (-12,9) circle[radius=2.2pt];

    \fill[BurntOrange] (12,1) circle[radius=2.2pt];
    \fill[Plum] (12,2) circle[radius=2.2pt];
    \fill[Plum] (12,3) circle[radius=2.2pt];

    % Threshold-invariant anchors at the four corners.
    \node[font=\large] at (-12,-12) {$\blacklozenge$};
    \node[font=\large] at (12,-12) {$\blacklozenge$};
    \node[font=\large] at (-12,12) {$\blacklozenge$};
    \node[font=\large] at (12,12) {$\blacklozenge$};

    \node[font=\scriptsize, anchor=north] at (0,-13.25)
      {$L=3,\ A=6,\ C=12$};
  \end{scope}
\end{tikzpicture}
\caption{The construction in dimension $d=2$.  In panel (a), coordinate $1$
orders the horizontal edge contexts bottom-to-top, whereas coordinate $2$
orders the vertical edge contexts right-to-left.  Panel (b) uses thresholds
$t_{00,10}=t_{00,01}=2$ and $t_{01,11}=t_{10,11}=1$.  Colored circles are the
fixed three-point edge chains, with colors indicating their labels for this
threshold choice; dashed marks show the four threshold gaps.  The corner
diamonds are threshold-invariant anchors.  In particular, the opposite pair
$B_{00},B_{11}$ is separated in coordinate $1$, while $B_{01},B_{10}$ is
separated in coordinate $2$.}
\label{fig:d2}
\end{figure}
